Noise Adaptor in Spiking Neural Networks

Recent strides in low-latency spiking neural network (SNN) algorithms have drawn significant interest, particularly due to their event-driven computing nature and fast inference capability. One of the most efficient ways to construct a low-latency SNN is by converting a pre-trained, low-bit artificial neural network (ANN) into an SNN. However, this conversion process faces two main challenges: First, converting SNNs from low-bit ANNs can lead to ``occasional noise" -- the phenomenon where occasional spikes are generated in spiking neurons where they should not be -- during inference, which significantly lowers SNN accuracy. Second, although low-latency SNNs initially show fast improvements in accuracy with time steps, these accuracy growths soon plateau, resulting in their peak accuracy lagging behind both full-precision ANNs and traditional ``long-latency SNNs'' that prioritize precision over speed. In response to these two challenges, this paper introduces a novel technique named ``noise adaptor.'' Noise adaptor can model occasional noise during training and implicitly optimize SNN accuracy, particularly at high simulation times $T$. Our research utilizes the ResNet model for a comprehensive analysis of the impact of the noise adaptor on low-latency SNNs. The results demonstrate that our method outperforms the previously reported quant-ANN-to-SNN conversion technique. We achieved an accuracy of 95.95\% within 4 time steps on CIFAR-10 using ResNet-18, and an accuracy of 74.37\% within 64 time steps on ImageNet using ResNet-50. Remarkably, these results were obtained without resorting to any noise correction methods during SNN inference, such as negative spikes or two-stage SNN simulations. Our approach significantly boosts the peak accuracy of low-latency SNNs, bringing them on par with the accuracy of full-precision ANNs. Code will be open source.

==> sec/6.tex <==
\section{Discussion and Limitation}
\subsection{Inference Accuracy at $T=1$}

Since a 1-bit activation-quantized ANN can be converted into an SNN with equivalent accuracy at the first simulation time step. This accuracy is usually much higher than 



, marking the peak accuracy achievable in comparison to other quantization settings. Notably, in the CIFAR-10 dataset, SNNs with p=2 demonstrate similar initial accuracy, suggesting their potential for high performance across various time steps. However, the ImageNet dataset shows a distinct trend, with all settings initially presenting low accuracy, improving gradually over time. These insights underscore the potential of designing SNNs with first-step accuracy on par with 1-bit ANNs, a promising direction for future research inspired by previous work with surrogate gradients




Considering the inference accuracy that an SNN can achieve at the first time steps, we note that when applying ANN-to-SNN conversion, a 1-bit activation-quantized ANN ($p=1$) can always be converted to an SNN with the same accuracy at the first simulation time step ($T=1$), and it should be the highest accuracy we can achieve, comparing to other activation quantization settings. 

Our results on CIFAR-10 show that the SNN with $p=2$ can also achieve similar accuracy as the one with $p=1$ at the first time step. This may be the reason that this network can achieve the best SNN accuracy in almost all time steps. However, we observe that in ImageNet, all settings have low accuracy at the first time steps, and the accuracy increases slowly but steadily with time steps.

Designing SNNs with accuracy in the first time step comparable to that of 1-bit ANNs is a topic we identify for future work. A previous study on surrogate gradients uses a 1-bit ANN to fine-tune with surrogate gradients. {add ref}


\subsection{Low-latency SNN does not mean low accuracy}

why high peak accuracy of low-latency SNNs important.
By this method, SNNs require considerably fewer simulation time steps, leading to faster AI computations. Moreover, the reduced simulation time steps reduce the need to retrieve model parameters, such as weights, thereby lowering Memory Access Cost (MAC) and fostering a more efficient AI system.

reducing the gap of low-latency SNNs and high-accuracy SNNs are important.

Also, it may avoid using multi model issue, we only need one model with full-precision model capability and fast response ability

\subsection{Noise correction vs. noise robustness}
The training of ANN is pivotal as it defines the characteristics of SNNs, especially in terms of latency and accuracy. 
we don't know different quantitation will help or not.

